Near Capacity Signaling over Fading Channels using Coherent Turbo Coded OFDM and Massive MIMO

The minimum average signal-to-noise ratio (SNR) per bit required for error-free transmission over a fading channel is derived, and is shown to be equal to that of the additive white Gaussian noise (AWGN) channel, which is $-1.6$ dB. Discrete-time algorithms are presented for timing and carrier synchronization, as well as channel estimation, for turbo coded multiple input multiple output (MIMO) orthogonal frequency division multiplexed (OFDM) systems. Simulation results show that it is possible to achieve a bit error rate of $10^{-5}$ at an average SNR per bit of 5.5 dB, using two transmit and two receive antennas. We then propose a near-capacity signaling method in which each transmit antenna uses a different carrier frequency. Using the near-capacity approach, we show that it is possible to achieve a BER of $2\times 10^{-5}$ at an average SNR per bit of just 2.5 dB, with one receive antenna for each transmit antenna. When the number of receive antennas for each transmit antenna is increased to 128, then a BER of $2\times 10^{-5}$ is attained at an average SNR per bit of 1.25 dB. In all cases, the number of transmit antennas is two and the spectral efficiency is 1 bit/transmission or 1 bit/sec/Hz. In other words, each transmit antenna sends 0.5 bit/transmission. It is possible to obtain higher spectral efficiency by increasing the number of transmit antennas, with no loss in BER performance, as long as each transmit antenna uses a different carrier frequency. The transmitted signal spectrum for the near-capacity approach can be restricted by pulse-shaping. In all the simulations, a four-state turbo code is used. The corresponding turbo decoder uses eight iterations. The algorithms can be implemented on programmable hardware and there is a large scope for parallel processing.

==> pap10_1_1.tex <==
%*******************************************************************************
\title{\textbf{\Large Near Capacity Signalling over Fading Channels using
Coherent Turbo Coded OFDM and Massive MIMO}}
\author{\IEEEauthorblockN{~\\[-0.4ex]\large K. Vasudevan\\[0.3ex]\normalsize}

\IEEEauthorblockA{Dept. of EE\\
                  IIT Kanpur\\
                  India\\
Email: {\tt vasu@iitk.ac.in}}
}
%*******************************************************************************
\maketitle
%*******************************************************************************
%\thispagestyle{empty}
%*******************************************************************************
\begin{abstract}
\boldmath
The minimum average signal-to-noise ratio (SNR) per bit required for error-free
transmission over a fading channel is derived, and is shown to be equal to
that of the additive white Gaussian noise (AWGN)
channel, which is $-1.6$ dB. Discrete-time algorithms are presented for
timing and carrier synchronization, as well as channel estimation, for
turbo coded multiple input multiple output (MIMO) orthogonal frequency
division multiplexed (OFDM) systems. Simulation results show that it is
possible to achieve a bit error rate of $10^{-5}$ at an SNR per bit of 5 dB,
using two transmit and receive antennas. If each transmit antenna
transmits at a different carrier frequency, then we show that it is possible
to achieve a BER of $10^{-5}$ at an SNR per bit of just 1.5 dB, with 16
receive antennas for each transmit antenna. When the number of
receive antennas for each transmit antenna is increased to 128, there is
no significant improvement in BER performance. In all cases, the number of
transmit antennas is two and the spectral efficiency is 1 bit/transmission.
In other words, each transmit antenna sends 0.5 bit/transmission. It is
possible to obtain higher spectral efficiencies by increasing the number of
transmit antennas, with no loss in BER performance, as long as each transmit
antenna uses a different carrier frequency.
In all the simulations, a four-state turbo code is used.
The algorithms can be implemented on programmable hardware and there is a
large scope for parallel processing.
\end{abstract}
%*******************************************************************************
\begin{IEEEkeywords}
MIMO; OFDM; coherent detection; matched filtering; turbo codes; frequency
selective Rayleigh fading; channel capacity; massive MIMO; spectral efficiency.
\end{IEEEkeywords}
%*******************************************************************************
\IEEEpeerreviewmaketitle
\bstctlcite{IEEEexample:BSTcontrol}
%*******************************************************************************
\section{Introduction}
\label{Sec:Intro}
We begin this article with an open question: what is the operating
signal-to-noise (SNR) per bit or $E_b/N_0$ of the present day mobile phones
\cite{Vasu_ICWMC2016,Vasudevan2015,DBLP:journals/corr/Vasudevan15a}?
The mobile phones indicate a
typical received signal strength of $-100$ dBm ($10^{-10}$ mW), however this
is not the SNR per bit. In order to seek the answer to this question, we first
briefly survey the state of affairs
in telecommunication engineering. There are two major players (a) the
academia and (b) the industry. The role of the academia is to develop new
concepts and to produce graduates and doctorates who are supposed to
join the industry and the university, in the form of engineers and teachers.
The role of the industry is to implement the new concepts, and bring out
products for the benefit of the common man. The new concepts proposed by the
academia are published in journals, conference proceedings and books, for the
purpose of dissemination. Now, some databases
have more than a million articles in telecommunications alone
\cite{Vasu_MAAZE_Edit16}. Assuming that
the million articles represent new ideas, let us ask a simple qustion:
how many of these ideas are used in a product, say a mobile phone? How many
ideas are being used in products without giving acknowledgement to its authors?
After all, nobody can see what is inside a mobile phone anyway.
How many publications are useless? It is time for uncomfortable
questions. Perhaps, instead of using the
citation index, we should have a ``product index'', with a binary value
0 or 1. A 1 indicates that the concept is used in a product, and
a 0 indicates otherwise. Of course, attaining any index is no problem for the
smart people.

Let us now turn our attention to the telecommunication graduates. Those
who join the industry, are compelled to leave in a few months, since they don't
know what they are doing. In fact, if we ask anyone in the industry ``what's
going on?'', the stock reply that one gets is: ``I don't know''. As a result,
many of the graduates end up in banks, stock markets and software companies,
where there is little use of what they have learnt in the university. The
graduates who still have their wits about them, go back to the universities
and hold on for dear life. Those who stay back in the industry are usually
the ones who don't know what they are doing, and the administrators (these
people are found everywhere). In fact, there is a saying:
%*******************************************************************************
\begin{flushleft}
{\it
Those who can, do.\\
Those who can't, teach.\\
Those who can't even teach, administrate.
}
\end{flushleft}
%*******************************************************************************
Perhaps, in the context of telecommunications engineering the above
saying needs to be modified to:
%*******************************************************************************
\begin{flushleft}
{\it
Those who can, teach.\\
Those who can't, do.\\
Those who can't even do, administrate.
}
\end{flushleft}
%*******************************************************************************
The administrators are actually quite powerful people. They work in the
form of ``sitting'' and ``standing'' committees. For example, the task of
a ``sitting'' selection committee is to get rid of outspoken people,
by identifying what they have {\it not\/} done in the last ten years.
Alternatively, one may have to work for the administrators or the powerful
people, to obtain a career advancement. Technically, this is called
``collaboration''.

To summarize, we seem to be still living in the Stone Age, where might is
right. One one hand, the authors are trying to outdo each other in writing
bigger and more complicated equations. In the absence of any real content for
publication there appears to be a common perception that big and complicated
equations are synonymous with quality. On the other hand, the demand for
genuine telecom engineers is far less than the supply.
Thus, the state of affairs of telecom engineering borders on absurdity. It is
time for the industry to open up and become more transparent. Just as
we have open access publications, we should also have open access products,
whose details of manufacture is accessible to all, e.g., the signal
processing algorithms that have gone into a mobile phone. Similarly,
with reference to the query raised in the beginning of this article,
it is necessary to specify the operating SNR per bit of the mobile phones.
After all, if the SNR per bit was such an important parameter in the
universities, why was it dropped by the industry? The university, on its part,
must restrict the number of publications. Whatever gets published should be
easily readable by all. It must be remembered that ideas come first and not
equations.
Having discussed the state of affairs, we now proceed to the literature
survey and the state of the art.

Future wireless communications, also called the 5th generation or 5G
\cite{6824752,7067426,7399671,7414384}, is supposed to involve not only people,
but also smart machines and devices, e.g., driverless cars, remotely
controlled washing machines, refrigerators, microwave ovens, robotic
surgeries in healthcare and so
on. Thus, we have to deal with an internet of things (IoT), which involves
device-to-human, human-to-device and device-to-device communications.
Depending on the application, there are different requirements on the
communication system. Critical applications like driverless cars and
robotic surgeries require low to medium bit rates, e.g., 0.1 -- 10 Mbps and low
latencies (the time taken to process the received information and send a
response back to the transmitter) of the order of a fraction of a millisecond.
Some applications like watching movies on a mobile phone require high bit
rates, e.g., 10 -- 1000 Mbps for high density and ultra high density (4k) video
and can tolerate high latency, of the order of a fraction of a second. Whatever
the application, the 5G wireless communication systems are expected to share
some common features like having a large number of transmit and receive
antennas also called massive multiple input multiple output (MIMO)
\cite{6375940,6415388,7294693,7601145} and the use of millimeter wave carrier
frequencies ($>$ 100 GHz) \cite{5783993,6387266,6515173,6882985,7574380},
to accommodate large bit-rates ($>$ 1 Gbps) and large number of users. In this
paper we deal with the physical layer of wireless systems that are also
applicable to 5G. The main topics addressed in this work are timing and
carrier synchronization, channel estimation, turbo codes and orthogonal
frequency division multiplexing (OFDM). Recall that OFDM converts a
frequency selective channel into a flat channel \cite{Vasu_Book10,Vasu_Book16}.

Channel characteristics in the THz frequency range and at 17 GHz for 5G indoor
wireless systems is studied in \cite{7511280,7725441}.
Channel estimation for massive MIMO assuming spatial correlation between
the receive antennas is considered in \cite{7752722,7760363}. In
\cite{7571183}, a MIMO channel estimator and beamformer is described.
Uplink channel estimation using compressive sensing for millimeter wave,
multiuser MIMO systems is considered in \cite{7727995,7752516}.
Error control coding for 5G is discussed in \cite{7593095,7565482}.

The main contribution of this paper is to
develop discrete-time algorithms for coherently detecting
multiple input, multiple output (MIMO),
orthogonal frequency division multiplexed (OFDM) signals, transmitted
over frequency selective Rayleigh fading channels. Carrier frequency offset and
additive white Gaussian noise (AWGN) are the other impairments considered in
this work. The minimum SNR per bit required for error-free transmission
over frequency selective MIMO fading channels is derived.
Finally we demonstrate how we can approach close to the channel capacity.
The capacity of single-user MIMO systems
under different assumptions about the channel impulse response (also
called the channel state information or CSI) and the statistics of the
channel impulse response (also called channel distribution information or CDI)
is discussed in \cite{1203154}. The capacity of MIMO Rayleigh fading
channels in the presence of interference and receive correlation is
discussed in \cite{4907090}. The low SNR capacity of MIMO fading channels
with imperfect channel state information is presented in \cite{6809207}.

Waveform design for spectral containment of the transmitted signal, is an
important aspect of wireless telecommunications, especially in the uplink,
where many users access a base station. We require that the signal from one
user does not interfere with the other user. This issue is addressed in
\cite{5753092,7022995,7469313,7509396,7510757,7564682,7566627,7744813,7744816,
7744817,7763353,7785158}.

To the best of our knowledge, other than the work in \cite{6663392},
which deals with turbo coded single input single output (SISO) OFDM, and
\cite{Vasudevan2015,DBLP:journals/corr/Vasudevan15a}, which deal with turbo
coded single input multiple output (SIMO) OFDM,
discrete-time algorithms for the coherent
detection of turbo coded MIMO OFDM systems have not been discussed earlier
in the literature. Simulations results for a $2\times 2$
turbo coded MIMO OFDM system indicate that a BER of $10^{-5}$, is obtained
at an SNR per bit of just 5.5 dB, which is a 2.5 dB improvement over the
performance given in \cite{Vasudevan2015}.

This paper is organized as follows. Section~\ref{Sec:Sys_Model} presents the
system model. The discrete-time algorithms and simulation results for the
coherent receiver are given in Section~\ref{Sec:Receiver}. Near-capacity
signalling is presented in Section~\ref{Sec:Near_Capacity}. Finally,
Section~\ref{Sec:Conclusions} concludes the paper.

